TSMixer: Lightweight MLP-Mixer Model for Multivariate Time Series Forecasting

Transformers have gained popularity in time series forecasting for their ability to capture long-sequence interactions. However, their high memory and computing requirements pose a critical bottleneck for long-term forecasting. To address this, we propose TSMixer, a lightweight neural architecture exclusively composed of multi-layer perceptron (MLP) modules for multivariate forecasting and representation learning on patched time series. Inspired by MLP-Mixer's success in computer vision, we adapt it for time series, addressing challenges and introducing validated components for enhanced accuracy. This includes a novel design paradigm of attaching online reconciliation heads to the MLP-Mixer backbone, for explicitly modeling the time-series properties such as hierarchy and channel-correlations. We also propose a novel Hybrid channel modeling and infusion of a simple gating approach to effectively handle noisy channel interactions and generalization across diverse datasets. By incorporating these lightweight components, we significantly enhance the learning capability of simple MLP structures, outperforming complex Transformer models with minimal computing usage. Moreover, TSMixer's modular design enables compatibility with both supervised and masked self-supervised learning methods, making it a promising building block for time-series Foundation Models. TSMixer outperforms state-of-the-art MLP and Transformer models in forecasting by a considerable margin of 8-60%. It also outperforms the latest strong benchmarks of Patch-Transformer models (by 1-2%) with a significant reduction in memory and runtime (2-3X). The source code of our model is officially released as PatchTSMixer in the HuggingFace. Model: https://huggingface.co/docs/transformers/main/en/model_doc/patchtsmixer Examples: https://github.com/ibm/tsfm/#notebooks-links

==> unused/experiment.tex <==
\subsection{Datasets}
We evaluate the performance of the proposed \tsm~model on 7 popular public datasets as depicted in the Table.~\ref{table:dataset}. These datasets have been extensively used in the literature~
\citep{autoformer}\citep{dlinear}~for benchmarking long-term multi-variate forecasting models.
\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{2pt}
\scalebox{0.85}{
\begin{tabular}{c|ccccccc}
\toprule  
Datasets & Weather  & Traffic & Electricity & ETTh1 & ETTh2 & ETTm1 & ETTm2 \\
\midrule  
Features & 21 & 862 & 321 & 7 & 7 & 7 & 7 \\
Timesteps & 52696 & 17544 & 26304 & 17420 & 17420 & 69680 & 69680 \\
\bottomrule 
\end{tabular}}
\caption{Statistics of popular datasets for benchmark.}
\label{table:dataset}
\end{table}


% We use the following naming conventions to represent a model configuration. ~\tsm can operate with 3 different backbone architectures: (i) ~\citsm: Channel Independent ~\tsm which only has inter-patch and intra-patch mixer in the MLP Mixer Layer and share weights across channels, (ii) ~\ictsm: Inter Channel ~\tsm which has inter-patch and intra-patch mixer in the MLP mixer layer (which shares weights across channels) and an explicit inter-channel mixer to capture the channel correlation. (iii) ~\vtsm 
\subsection{Model Naming Convention}
A ~\tsm~ Model variant is represented using the naming convention ${"BackboneType"}$-\tsm(${"Enhancements"}$).
${"BackboneType"}$ can either be Vanilla (\van) or Channel Independent (\ci) or Inter Channel (\ic).
${"Enhancements"}$ can be a combination of Gated Attention (\ga), Hierarchy Reconciliation head (\hr
) and/or Cross-channel Reconciliation head (\cc). Common Variants are as follows:
\begin{itemize}
    \item \textbf{~\ci-\tsm}: Channel Independent ~\tsm~ with no enhancements
    \item \textbf{~\tsmgh}: Channel Independent ~\tsm~ with Gated Attention and Hierarchy Reconciliation head
    \item \textbf{~\tsmghc}: Channel Independent ~\tsm~ with Gated Attention, Hierarchy and Cross-Channel Reconciliation head
    \item \textbf{~\tsmb}: Best of top performing ~\tsm~variants [i.e. ~\tsmgh~ and ~\tsmghc]
    \item \textbf{\vtsm}: Vanilla ~\tsm
    \item \textbf{\ictsm}: Inter-Channel ~\tsm
\end{itemize}
Other model variants can be formed using the same naming convention.

\subsection{Experimental setting}
By default, the following data and model configuration is used: Input Sequence length $sl$ = 512, Patch length $pl$ = 16, Stride $s$ = 8, Batch size $b$ = 8, Forecast sequence length $fl \in \{96, 192, 336, 720\}$, Number of MLP Mixer layers $nl$ = 8, Hidden feature size $hf$ = 32, Expansion feature size $ef$ = 64 and Dropout $do$ = 0.1. Training is performed in a distributed fashion with 8 GPUs, 10 CPUs and 100 GB of memory. For ETT datasets, we use a lower hardware and model configuration with high dropout to avoid over-fitting, as the dataset is relatively small($nl$ = 3, $do$ = 0.7, $ngpus$ = 1). Supervised workflows are trained with 100 epochs and in self-supervised workflows, we first pretrain the backbone with 100 epochs and in the finetuning phase - we freeze the backbone for the first 20 epochs to bootstrap the head and then we finetune the entire network (backbone + head) for the next 100 epochs. Since overlapping patches have to be avoided in self-supervised workflows, we use the same patch length and stride(i.e. $pl$ = 8, $s$ = 8) for self-supervised workflows.  Every experiment is executed with 5 seeds (42-46) and the mean result is reported. Standard deviation is also reported for the primary results. We use MSE and MAE as the standard error metrics to report the results. 




% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|}
%     \hline
%         Metric & Data & Patch TST & CI-TSMixer (Imp) & CI-TSMixer(G,H) (Imp) & CI-TSMixer(G,H,CC) (Imp) \\ \hline
%         MACs(T) & Electricity & 147.879 & 37.062 (4X) & 46.44 (3.2X) & 48.566 (3X) \\ \hline
%         MACs(T) & Traffic & 260.367 & 65.25 (4X) & 81.77 (3.2X) & 91.78 (2.8X) \\ \hline
%         MACs(T) & Weather & 19.709 & 4.94 (4X) & 6.19 (3.2X) & 6.21 (3.2X) \\ \hline
%         PARAMETERS (M) & Electricity & 1.174 & 0.348 (3.4X) & 0.4 (2.9X) & 1.648 (0.7X) \\ \hline
%         PARAMETERS (M) & Traffic & 1.174 & 0.348 (3.4X) & 0.4 (2.9X) & 9.33 (0.1X) \\ \hline
%         PARAMETERS (M) & Weather & 1.174 & 0.348 (3.4X) & 0.4 (2.9X) & 0.405 (2.9X) \\ \hline
%         EPOCH TIME (min) & Electricity & 36.22 & 15.56 (2.3X) & 20.43 (1.8X) & 20.5 (1.8X) \\ \hline
%         EPOCH TIME (min) & Traffic & 64.04 & 27.49 (2.3X) & 36.08 (1.8X) & 36.51 (1.8X) \\ \hline
%         EPOCH TIME (min) & Weather & 5.2 & 3.08 (1.7X) & 4.13 (1.3X) & 4.17 (1.2X) \\ \hline
%         MAX MEMORY (GB) & Electricity & 6.14 & 2.25 (2.7X) & 2.9 (2.1X) & 2.94 (2.1X) \\ \hline
%         MAX MEMORY (GB) & Traffic & 8.24 & 3.03 (2.7X) & 3.89 (2.1X) & 4.15 (2X) \\ \hline
%         MAX MEMORY (GB) & Weather & 0.451 & 0.165 (2.7X) & 0.21 (2.1X) & 0.211 (2.1X) \\ \hline
%     \end{tabular}
% \end{table}

\subsection{SOTA Benchmarks}
We categorize SOTA benchmarks into the following categories: 
\begin{itemize}
    \item \textbf{Standard Transformer based forecasting benchmarks}: FEDformer~\cite{fedformer}, Autoformer\cite{autoformer} and Informer ~\cite{informer}. We exclude Pyraformer~\cite{pyraformer} and LogTrans~\cite{logtrans} considering their inferior performance wrt. FEDformer ~\cite{fedformer}.
    \item \textbf{Patch Transformer based forecasting benchmark:} \\ PatchTST~\cite{patchtst} 
    \item \textbf{MLP and Non-Transformer based forecasting benchmarks: }DLinear~\cite{dlinear}, LightTS~\cite{lightts} and S4~\cite{s4}
    \item \textbf{Self-supervised forecasting benchmarks:} BTSF~\cite{btsf}, TNC~\cite{tnc}, TS-TCC~\cite{ts-tcc}, CPC~\cite{cpc}, and TS2Vec~\cite{ts2vec}
    
\end{itemize}

 

\begin{table*}[htb]
        % \small
	\centering
	\resizebox{\linewidth}{!}{
		  \begin{tabular}{cc|c|cc|cc|cc|cc|cc|ccc}
            \cline{2-15}
			&\multicolumn{2}{c|}{Models} & \multicolumn{2}{c}{\textbf{\citsm-Best}} & \multicolumn{2}{c|}{DLinear} & \multicolumn{2}{c|}{PatchTST}& \multicolumn{2}{c|}{FEDformer}& \multicolumn{2}{c|}{Autoformer}& \multicolumn{2}{c}{Informer} \\
			\cline{2-15}
			&\multicolumn{2}{c|}{Metric}&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE\\
			\cline{2-15}
            &\multirow{4}*{\rotatebox{90}{ETTH1}} & 96 & \textbf{0.368$\pm$0.001} & \textbf{0.398$\pm$0.001} & 0.375 & \uline{0.399} & \uline{0.37} & 0.4 & 0.376 & 0.419 & 0.449 & 0.459 & 0.865 & 0.713 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.399$\pm$0.002} & \uline{0.418$\pm$0.001} & \uline{0.405} & \textbf{0.416} & 0.413 & 0.429 & 0.42 & 0.448 & 0.5 & 0.482 & 1.008 & 0.792 \\ 
            &\multicolumn{1}{c|}{} & 336 & \textbf{0.421$\pm$0.004} & \textbf{0.436$\pm$0.003} & 0.439 & 0.443 & \uline{0.422} & \uline{0.44} & 0.459 & 0.465 & 0.521 & 0.496 & 1.107 & 0.809 \\ 
            &\multicolumn{1}{c|}{} & 720 & \textbf{0.444$\pm$0.003} & \textbf{0.467$\pm$0.002} & 0.472 & 0.49 & \uline{0.447} & \uline{0.468} & 0.506 & 0.507 & 0.514 & 0.512 & 1.181 & 0.865 \\ 
            \cline{2-15} 
            &\multirow{4}*{\rotatebox{90}{ETTH2}} & 96 & \uline{0.276$\pm$0.006} & \textbf{0.337$\pm$0.003} & 0.289 & \uline{0.353} & \textbf{0.274} & \textbf{0.337} & 0.346 & 0.388 & 0.358 & 0.397 & 3.755 & 1.525 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.33$\pm$0.003} & \textbf{0.374$\pm$0.001} & 0.383 & 0.418 & \uline{0.341} & \uline{0.382} & 0.429 & 0.439 & 0.456 & 0.452 & 5.602 & 1.931 \\ 
            &\multicolumn{1}{c|}{} & 336 & \uline{0.357$\pm$0.001} & \uline{0.401$\pm$0.002} & 0.448 & 0.465 & \textbf{0.329} & \textbf{0.384} & 0.496 & 0.487 & 0.482 & 0.486 & 4.721 & 1.835 \\ 
            &\multicolumn{1}{c|}{} & 720 & \uline{0.395$\pm$0.003} & \uline{0.436$\pm$0.003} & 0.605 & 0.551 & \textbf{0.379} & \textbf{0.422} & 0.463 & 0.474 & 0.515 & 0.511 & 3.647 & 1.625 \\ 
            \cline{2-15} 
            &\multirow{4}*{\rotatebox{90}{ETTM1}} & 96 & \textbf{0.291$\pm$0.002} & \uline{0.346$\pm$0.002} & 0.299 & \textbf{0.343} & \uline{0.293} & \uline{0.346} & 0.379 & 0.419 & 0.505 & 0.475 & 0.672 & 0.571 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.333$\pm$0.002} & \uline{0.369$\pm$0.002} & \uline{0.335} & \textbf{0.365} & \textbf{0.333} & 0.37 & 0.426 & 0.441 & 0.553 & 0.496 & 0.795 & 0.669 \\ 
            &\multicolumn{1}{c|}{} & 336 & \textbf{0.365$\pm$0.005} & \textbf{0.385$\pm$0.004} & \uline{0.369} & \uline{0.386} & \uline{0.369} & 0.392 & 0.445 & 0.459 & 0.621 & 0.537 & 1.212 & 0.871 \\ 
            &\multicolumn{1}{c|}{} & 720 & \textbf{0.416$\pm$0.002} & \textbf{0.413$\pm$0.001} & \uline{0.425} & 0.421 & \textbf{0.416} & \uline{0.42} & 0.543 & 0.49 & 0.671 & 0.561 & 1.166 & 0.823 \\ 
            \cline{2-15} 
            &\multirow{4}*{\rotatebox{90}{ETTM2}} & 96 & \textbf{0.164$\pm$0.002} & \textbf{0.255$\pm$0.002} & 0.167 & 0.26 & \uline{0.166} & \uline{0.256} & 0.203 & 0.287 & 0.255 & 0.339 & 0.365 & 0.453 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.219$\pm$0.002} & \textbf{0.293$\pm$0.002} & 0.224 & 0.303 & \uline{0.223} & \uline{0.296} & 0.269 & 0.328 & 0.281 & 0.34 & 0.533 & 0.563 \\ 
            &\multicolumn{1}{c|}{} & 336 & \textbf{0.273$\pm$0.003} & \textbf{0.329$\pm$0.003} & 0.281 & \uline{0.342} & \uline{0.274} & \textbf{0.329} & 0.325 & 0.366 & 0.339 & 0.372 & 1.363 & 0.887 \\ 
            &\multicolumn{1}{c|}{} & 720 & \textbf{0.358$\pm$0.002} & \textbf{0.38$\pm$0.001} & 0.397 & 0.421 & \uline{0.362} & \uline{0.385} & 0.421 & 0.415 & 0.433 & 0.432 & 3.379 & 1.338 \\ 
            \cline{2-15} 
            &\multirow{4}*{\rotatebox{90}{Electricity}} & 96 & \textbf{0.129$\pm$1e-4} & \uline{0.224$\pm$0.001} & \uline{0.14} & 0.237 & \textbf{0.129} & \textbf{0.222} & 0.193 & 0.308 & 0.201 & 0.317 & 0.274 & 0.368 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.146$\pm$0.001} & \uline{0.242$\pm$1e-4} & 0.153 & 0.249 & \uline{0.147} & \textbf{0.24} & 0.201 & 0.315 & 0.222 & 0.334 & 0.296 & 0.386 \\ 
            &\multicolumn{1}{c|}{} & 336 & \textbf{0.158$\pm$0.001} & \textbf{0.256$\pm$0.001} & 0.169 & 0.267 & \uline{0.163} & \uline{0.259} & 0.214 & 0.329 & 0.213 & 0.338 & 0.3 & 0.394 \\ 
            &\multicolumn{1}{c|}{} & 720 & \textbf{0.186$\pm$0.001} & \textbf{0.282$\pm$0.001} & 0.203 & 0.301 & \uline{0.197} & \uline{0.29} & 0.246 & 0.355 & 0.254 & 0.361 & 0.373 & 0.439 \\ 
            \cline{2-15} 
            &\multirow{4}*{\rotatebox{90}{Traffic}} & 96 & \textbf{0.356$\pm$0.002} & \textbf{0.248$\pm$0.002} & 0.41 & 0.282 & \uline{0.36} & \uline{0.249} & 0.587 & 0.366 & 0.613 & 0.388 & 0.719 & 0.391 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.377$\pm$0.003} & \uline{0.257$\pm$0.002} & 0.423 & 0.287 & \uline{0.379} & \textbf{0.256} & 0.604 & 0.373 & 0.616 & 0.382 & 0.696 & 0.379 \\ 
            &\multicolumn{1}{c|}{} & 336 & \textbf{0.385$\pm$0.002} & \textbf{0.262$\pm$0.001} & 0.436 & 0.296 & \uline{0.392} & \uline{0.264} & 0.621 & 0.383 & 0.622 & 0.337 & 0.777 & 0.42 \\ 
            &\multicolumn{1}{c|}{} & 720 & \textbf{0.424$\pm$0.001} & \textbf{0.283$\pm$0.001} & 0.466 & 0.315 & \uline{0.432} & \uline{0.286} & 0.626 & 0.382 & 0.66 & 0.408 & 0.864 & 0.472 \\ 
            \cline{2-15} 
            &\multirow{4}*{\rotatebox{90}{Weather}} & 96 & \textbf{0.146$\pm$0.001} & \textbf{0.197$\pm$0.002} & 0.176 & 0.237 & \uline{0.149} & \uline{0.198} & 0.217 & 0.296 & 0.266 & 0.336 & 0.3 & 0.384 \\ 
            &\multicolumn{1}{c|}{} & 192 & \textbf{0.191$\pm$0.001} & \textbf{0.24$\pm$0.001} & 0.22 & 0.282 & \uline{0.194} & \uline{0.241} & 0.276 & 0.336 & 0.307 & 0.367 & 0.598 & 0.544 \\ 
            &\multicolumn{1}{c|}{} & 336 & \textbf{0.243$\pm$0.001} & \textbf{0.279$\pm$0.002} & 0.265 & 0.319 & \uline{0.245} & \uline{0.282} & 0.339 & 0.38 & 0.359 & 0.395 & 0.578 & 0.523 \\ 
            &\multicolumn{1}{c|}{} & 720 & \uline{0.316$\pm$0.001} & \textbf{0.333$\pm$0.002} & 0.323 & 0.362 & \textbf{0.314} & \uline{0.334} & 0.403 & 0.428 & 0.419 & 0.428 & 1.059 & 0.741 \\ 
            \cline{2-15} 
            &\multicolumn{4}{c|}{\makecell{\textbf{\citsm-Best} \textbf{\% improvement}}}& \textbf{8\%} & \textbf{6.8\%}& \textbf{0.7\%} & \textbf{0.4\%} & \textbf{22.9\%} & \textbf{18.2\%} & \textbf{30.1\%} & \textbf{22.7\%} & \textbf{64\%} & \textbf{50.3\%} \\
            \cline{2-15} 
		\end{tabular}
	}
	\caption{Supervised Long-term multivariate forecasting. The best results are in bold and the second best is underlined.}
	\label{tab:supervised}
\end{table*}


\subsection{Supervised Multivariate Forecasting}
In Table.~\ref{tab:supervised}, we compare and contrast the \tsm~ Best variant (i.e. ~\tsmb) with existing SOTA benchmarks on the supervised multivariate forecasting problem. Since MSE and MAE report similar relative characteristics wrt. benchmarks, we explain all our results using the MSE metric. ~\tsm~ outperforms standard transformer and MLP models by a significant margin (DLinear - 8\%, FEDformer -  23\%, Autoformer - 30\% and Informer - 64\%). Since LightTS and S4 report results in a different experiment setting, we highlight their results in Appendix (Table.~\ref{tab:lightts}), where \tsm~ outperforms LightTS and S4 by 33\% and 66\%. PatchTST (which refers to PatchTST/64 in ~\cite{patchtst}) is the strongest baseline, which \tsm~ marginally beats by $\sim$1\%. However, ~\tsm~ achieves this marginal improvement over PatchTST with a significant performance improvement wrt. training time and memory as explained in the next section. For more details on drill-down results with respect to individual best~\tsm variants [i.e. ~\tsmgh~ and ~\tsmghc], refer to Appendix (Table.~\ref{tab:ga_hc-ab1})



\subsection{Memory \& Training Time Benchmark}
\label{sec:speedup}
In  Table.~\ref{tab:speedup}, we highlight the speed-up comparison of ~\tsm~ over PatchTST. To report the training time and memory usage improvements, we capture the following performance metrics: (i) Multiply-Add cumulative operations on the entire data per epoch (macs), (ii) Number of model parameters (nparams), (iii) Single epoch time and (iv) Peak GPU memory reached during a training run (max memory). Both ~\tsm~ and PatchTST models are trained in a single GPU node with the same hardware configuration. To ensure fairness in comparison, we use the exact model parameters of PatchTST and ~\tsm~ which were used in the error metric comparison reported in Table.~\ref{tab:supervised}. Also, to capture the exact metrics without extra overheads, we avoid distributed training in this experiment. Table.~\ref{tab:speedup} captures the average improvement of ~\tsm~ over PatchTST for each performance metric across the 3 big datasets. Since ~\citsm~ avoids the heavy processing multi-head self-attention blocks, it significantly reduces the average macs by 4X, nparams \& max memory by 3X, and epoch time \footnote{Macs and epoch time are highly correlated and in general create a similar relative impact across models. However, since PatchTST involves high parallelism across the attention heads, we observe a different relative impact wrt. macs and epoch time.} by 2X.  Even after enabling Gated Attention and Hierarchy reconciliation, ~\tsmgh~ still shows a good reduction in macs \& nparams (by 3X), and epoch time \& max memory (by 2X). It is important to note that, when cross-channel reconciliation is enabled [i.e ~\tsmghc], the number of parameters scales very high in ~\tsm~ as compared to PatchTST. The reason is, the number of parameters in the cross-channel reconciliation head is dependent on the number of channels in the dataset which leads to this scaling effect. For Ex. Since Electricity and Traffic have a very high number of channels(i.e. 321 and 862), the number of parameters of the model also scales up, whereas weather (with only 21 channels) didn't show any such scaling effect. Even PatchTST will show similar scaling effect if channel correlation is enabled in it. However, even with increased parameters, ~\tsmghc~ still shows a notable reduction wrt. macs (by 3X) and epoch time \& max memory (by 2X).  The reason is, parameter scaling affects only the reconciliation head and not the backbone which primarily constitutes the total training time and memory. Thus, ~\tsm~ and its variants can easily produce improved results over PatchTST with extremely less training time and memory utilization.   



\begin{table}
\centering
\setlength{\tabcolsep}{1.5pt}
\scalebox{0.9}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline  
Metric & Data & \makecell{Patch\\TST} & \multicolumn{2}{c|}{\makecell{\citsm\\(Avg. Imp)}} & \multicolumn{2}{c|}{\makecell{\citsm\\(\ga,\hr)\\(Avg. Imp)}} & \multicolumn{2}{c}{\makecell{\citsm\\(\ga,\hr,\cc)\\(Avg. Imp)}}  \\
\hline
\multirow{3}{*}{\makecell{MACs\\(T)}}  & Electricity & 147.879 & 37.062 &\multirow{3}*{\rotatebox{90}{\textbf{(4X)}}} & 46.44 &\multirow{3}*{\rotatebox{90}{\textbf{(3.2X)}}} & 48.566 &\multirow{3}*{\rotatebox{90}{\textbf{(3X)}}} \\ 
& Traffic & 260.367 & 65.25 &\multicolumn{1}{c|}{} & 81.77 &\multicolumn{1}{c|}{} & 91.78 &\multicolumn{1}{c}{} \\ 
& Weather & 19.709 & 4.94 &\multicolumn{1}{c|}{} & 6.19 &\multicolumn{1}{c|}{} & 6.21 &\multicolumn{1}{c}{} \\ \hline

\multirow{3}{*}{\makecell{NPARAMS \\ (M)}}   & Electricity & 1.174 & 0.348 &\multirow{3}*{\rotatebox{90}{\textbf{(3.4X)}}} & 0.4 &\multirow{3}*{\rotatebox{90}{\textbf{(2.9X)}}} & 1.648 &\multirow{3}*{\rotatebox{90}{\textbf{(1.2X)}}} \\ 
 & Traffic & 1.174 & 0.348 &\multicolumn{1}{c|}{} & 0.4 &\multicolumn{1}{c|}{} & 9.33 &\multicolumn{1}{c}{} \\ 
 & Weather & 1.174 & 0.348 &\multicolumn{1}{c|}{} & 0.4 &\multicolumn{1}{c|}{} & 0.405 &\multicolumn{1}{c}{} \\ \hline

\multirow{3}{*}{\makecell{EPOCH \\ TIME \\(min)}}  & Electricity & 36.22 & 15.56  &\multirow{3}*{\rotatebox{90}{\textbf{(2X)}}} & 20.43 &\multirow{3}*{\rotatebox{90}{\textbf{(1.6X)}}} & 20.5 &\multirow{3}*{\rotatebox{90}{\textbf{(1.5X)}}} \\ 
 & Traffic & 64.04 & 27.49 &\multicolumn{1}{c|}{} & 36.08 &\multicolumn{1}{c|}{} & 36.51 &\multicolumn{1}{c}{} \\ 
 & Weather & 5.2 & 3.08 &\multicolumn{1}{c|}{} & 4.13 &\multicolumn{1}{c|}{} & 4.17 &\multicolumn{1}{c}{} \\ \hline
 
\multirow{3}{*}{\makecell{MAX  \\ MEMORY \\ (GB)}}  & Electricity & 6.14 & 2.25 &\multirow{3}*{\rotatebox{90}{\textbf{(2.7X)}}} & 2.9 &\multirow{3}*{\rotatebox{90}{\textbf{(2.1X)}}} & 2.94 &\multirow{3}*{\rotatebox{90}{\textbf{(2X)}}} \\ 
& Traffic & 8.24 & 3.03 &\multicolumn{1}{c|}{} & 3.89 &\multicolumn{1}{c|}{} & 4.15 &\multicolumn{1}{c}{} \\ 
& Weather & 0.451 & 0.165 &\multicolumn{1}{c|}{} & 0.21 &\multicolumn{1}{c|}{} & 0.211 &\multicolumn{1}{c}{} \\ \hline
\end{tabular}}
\caption{Speed-Up Comparison}
\label{tab:speedup}
\end{table}

\subsection{Effect of CI, Gated Attention and Hierarchy Reconciliation over Vanilla}
Table.~\ref{tab:ci_ga_hr} depicts the improvements of various enhancements components in ~\tsm~ over ~\vtsm~ using datasets ETTH1, ETTM1, and Weather. For results on the complete datasets, refer to the Appendix (Table.~\ref{tab:ga_hc-ab1}). ~\vtsm~ represents the vanilla model where all channels are flattened and processed together (similar to vision mlp mixer models). ~\citsm~ outperforms ~\vtsm~ by 9.5\% by introducing channel independence in the backbone instead of channel flattening. By further adding Gated Attention (G) and Hierarchy Reconciliation (H) together [i.e. ~\tsmgh], we observe an additional 2\% improvement leading to a total of 11.5\% improvement wrt. ~\vtsm. On the complete dataset (Appendix Table.~\ref{tab:ga_hc-ab1}), we observe that ~\tsmgh~ outperforms ~\vtsm~ by 19.3\%. It is important to note that, adding G and H together leads to more stable improvements wrt. ~\citsm~ as compared to just adding G or H.  



\begin{table}
\centering
\setlength{\tabcolsep}{2pt}
\scalebox{0.98}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline  
& \makecell{FL} & \makecell{V-\\\tsm} & \makecell{CI-\\\tsm} & \makecell{\citsm\\(\ga)} & \makecell{\citsm\\(\hr)} & \makecell{\citsm\\(\ga,\hr)}  \\
\hline
\multirow{4}{*}{\rotatebox{90}{ETTH1}} & 96 & 0.449 & 0.375 & 0.375 & 0.377 & \textbf{0.368} \\ 
& 192 & 0.485 & 0.411 & 0.408 & 0.41 & \textbf{0.399} \\ 
& 336 & 0.504 & 0.437 & 0.433 & 0.431 & \textbf{0.421} \\ 
& 720 & 0.573 & 0.465 & 0.454 & 0.457 & \textbf{0.444} \\ \hline

\multirow{4}{*}{\rotatebox{90}{ETTM1}} & 96 & 0.328 & 0.305 & \textbf{0.296} & 0.301 & 0.297 \\ 
& 192 & 0.372 & 0.336 & 0.334 & 0.338 & \textbf{0.333} \\ 
& 336 & 0.405 & 0.375 & 0.366 & 0.376 & \textbf{0.365} \\ 
& 720 & 0.457 & 0.425 & 0.419 & 0.422 & \textbf{0.416} \\ \hline

\multirow{4}{*}{\rotatebox{90}{Weather}}  & 96 & 0.159 & 0.15 & 0.149 & 0.151 & \textbf{0.148} \\ 
& 192 & 0.207 & 0.195 & 0.195 & 0.195 & \textbf{0.193} \\ 
& 336 & 0.256 & 0.246 & 0.246 & 0.246 & \textbf{0.243} \\ 
& 720 & 0.33 & 0.323 & 0.317 & 0.321 & \textbf{0.317} \\ \hline
\multicolumn{3}{c|}{ \makecell{\textbf{\% improvement} \\ \textbf{over \vtsm}}} & \textbf{9.5\%}	& \textbf{10.5\%} & \textbf{10\%} & \textbf{11.5\%} \\ \hline
% &\multicolumn{3}{c|}{\makecell{\textbf{\citsm-Best} & \textbf{9.372}}	& \textbf{10.421} & \textbf{9.656} & \textbf{11.352} \\ \hline
\end{tabular}}
\caption{Effect of CI, Gated Attention and Hierarchy Reconciliation over Vanilla~\tsm. MSE mean reported.}
\label{tab:ci_ga_hr}
\end{table}

\subsection{Analyzing various channel mixing techniques}
In Table.~\ref{tab:channel_table}, we compare and contrast various channel-mixing techniques in ~\tsm~ using datasets ETTH1, ETTH2 and Weather. For results on the complete dataset, refer to the Appendix (Table.~\ref{tab:cc-detail}). In summary, ~\citsm~ outperforms \vtsm~ by 11.5\% and by adding cross-channel reconciliation head (cc), accuracy further improves by 2\% leading to an overall improvement of 13.5\% for \citsm(\ga,\cc-Best). Context Length ($cl$) is an important hyperparameter in the CC head that decides the surrounding context space across channels to enable reconciliation and this parameter has to be decided based on the underlying data characteristics. For this experiment, we ran $cl$ from 1 to 5 and selected the best which is depicted as \citsm(\ga,\cc-Best) in Table.~\ref{tab:channel_table}. For drill-down results on various context lengths, refer to the Appendix(Table.~\ref{tab:cc-detail}). Also, we observe from Table.~\ref{tab:channel_table} that channel Independence in the backbone (i.e. ~\citsm) performs better as compared to the inter-channel mixer (i.e. ~\ictsm). From an architectural point, another advantage of having channel independence in the backbone is that, it greatly helps in pretraining the models with multiple datasets with varying channel counts (as explained in later sections). This cannot be achieved with an inter-channel or vanilla backbone. Hence, having a channel-independent backbone with a cross-channel reconciliation head enables effective capture of cross-channel correlations while giving the flexibility to the backbone to pretrain with multiple datasets with varying channel counts.


\begin{table}
\centering
\setlength{\tabcolsep}{2pt}
\scalebox{1.1}{
\begin{tabular}{c|c|c|c|c|c}
\hline  
& \makecell{FL} & \makecell{V-\tsm} & \makecell{CI-\tsm} & \makecell{IC-\tsm} & \makecell{\citsm\\(\ga,\cc-Best)}  \\
\hline
\multirow{4}{*}{\rotatebox{90}{ETTH1}} & 96 & 0.449 & 0.375 & 0.379 & \textbf{0.373} \\ 
    & 192 & 0.485 & 0.411 & 0.416  & \textbf{0.407} \\ 
    & 336 & 0.504 & 0.437 & 0.437  & \textbf{0.43} \\ 
     & 720 & 0.573 & 0.465 & 0.471  & \textbf{0.454} \\  \hline
\multirow{4}{*}{\rotatebox{90}{ETTH2}} & 96 & 0.369 & 0.284 & 0.291  & \textbf{0.269} \\
     & 192 & 0.391 & 0.353 & 0.345  & \textbf{0.33} \\ 
     & 336 & 0.403 & 0.365 & 0.361  & \textbf{0.359} \\ 
     & 720 & 0.475 & 0.406 & 0.419  & \textbf{0.393 }\\  \hline
\multirow{4}{*}{\rotatebox{90}{Weather}} & 96 & 0.159 & 0.15 & 0.15  & \textbf{0.146} \\
     & 192 & 0.207 & 0.195 & 0.196  & \textbf{0.194} \\ 
     & 336 & 0.256 & \textbf{0.246} & 0.248  & \textbf{0.246} \\ 
     & 720 & 0.33 & 0.323 & 0.338 & \textbf{0.317} \\  \hline


\multicolumn{3}{c|}{ \makecell{\textbf{\% improvement} \\ \textbf{over \vtsm}}} & \textbf{11.5\%}	& \textbf{10.7\%}  & \textbf{13.5\%} \\ \hline
% &\multicolumn{3}{c|}{\makecell{\textbf{\citsm-Best} & \textbf{9.372}}	& \textbf{10.421} & \textbf{9.656} & \textbf{11.352} \\ \hline
\end{tabular}}
\caption{Comparison of various channel mixing techniques. MSE mean reported.}
\label{tab:channel_table}
\end{table}


\begin{table}
\centering
\setlength{\tabcolsep}{2pt}
\scalebox{0.98}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline  
& \makecell{FL} & \makecell{CI-\tsm\\-Best} & \makecell{PatchTST} & \makecell{BTSF} & \makecell{TNC} & \makecell{TS-TCC} & \makecell{CPC}  \\
\hline
\multirow{5}*{\rotatebox{90}{ETTH1}} & 24.0 & \textbf{0.314} & \uline{0.322} & 0.541 & 0.632 & 0.653 & 0.687 \\ 
\multicolumn{1}{c|}{} & 48.0 & \textbf{0.343} & \uline{0.354} & 0.613 & 0.705 & 0.72 & 0.779 \\ 
\multicolumn{1}{c|}{} & 168.0 & \textbf{0.397} & \uline{0.419} & 0.64 & 1.097 & 1.129 & 1.282 \\ 
\multicolumn{1}{c|}{} & 336.0 & \textbf{0.424} & \uline{0.445} & 0.864 & 1.454 & 1.492 & 1.641 \\ 
\multicolumn{1}{c|}{} & 720.0 & \textbf{0.453} & \uline{0.487} & 0.993 & 1.604 & 1.603 & 1.803 \\ 
\hline 

\multirow{5}*{\rotatebox{90}{Weather}} & 24.0 & \uline{0.088} & \textbf{0.087} & 0.324 & 0.484 & 0.572 & 0.647 \\ 
\multicolumn{1}{c|}{} & 48.0 & \uline{0.114} & \textbf{0.113} & 0.366 & 0.608 & 0.647 & 0.72 \\ 
\multicolumn{1}{c|}{} & 168.0 & \textbf{0.177} & \uline{0.178} & 0.543 & 1.081 & 1.117 & 1.351 \\ 
\multicolumn{1}{c|}{} & 336.0 & \textbf{0.241} & \uline{0.244} & 0.568 & 1.654 & 1.783 & 2.019 \\ 
\multicolumn{1}{c|}{} & 720.0 & \textbf{0.319} & \uline{0.321} & 0.601 & 1.401 & 1.85 & 2.109 \\ 
\hline 

\multicolumn{3}{c|}{ \makecell{\textbf{\citsm-Best} \\ \textbf{\% improvement}}} & \textbf{2.3\%}	& \textbf{54.2\%} & \textbf{71.7\%} & \textbf{73.3\%} & \textbf{75.8\%} \\ \hline
% &\multicolumn{3}{c|}{\makecell{\textbf{\citsm-Best} & \textbf{9.372}}	& \textbf{10.421} & \textbf{9.656} & \textbf{11.352} \\ \hline
\end{tabular}}
\caption{Self-Supervised Multivariate forecasting with pretrain and finetune workflows. MSE mean reported.}
\label{tab:fm_1}
\end{table}


\subsection{Self-Supervised Multivariate forecasting}
In Table.~\ref{tab:fm_1}, we compare and contrast the forecasting results achieved via self-supervised pretrain and finetune workflows on datasets ETTH1 and Weather. In this workflow, the TSMixer backbone is first pretrained to learn a generic patch representation, and then the entire network (backbone + head) is finetuned for the forecasting task. By training ~\tsm~ with this training approach, we observe from Table.~\ref{tab:fm_1} that ~\tsmb~ achieves a significant improvement (50-70\% margin) with existing forecasting benchmarks learned via self-supervision (or representation learning) techniques (such as BFSF, TNC, TS-TCC, CPC). Similar trends were also observed with TS2Vec which is depicted separately in Appendix(Table.~\ref{tab:ab_ts2vec}) due to different experimental settings. ~\tsmb~ also beats self-supervised PatchTST by a notable margin of 2\%. However, as explained in Section.~\ref{sec:speedup}, we achieve this improvement over PatchTST with a very significant reduction in time and memory. A more detailed analysis between self-supervised ~\tsm~ and PatchTST with all the considered 3 big datasets is explained in the next section. 


% \begin{table*}[t]
%     % \setlength{\tabcolsep}{5pt}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%         \toprule
        
%         & FL & \makecell{\citsm-\\Overall-Best (SS)} &  \multicolumn{3}{c|}{\makecell{\citsm-Best (SS) \\ Model Size: Default}}& \multicolumn{3}{c|}{\makecell{\citsm-Best (SS) \\ Model Size: Big}} & \makecell{PatchTST \\ (SS)}& \makecell{\citsm-\\Best} \\ \hline

%         & & & SAME & ALL & TL & SAME & ALL & TL &  & Supervised\\ \hline
%         \multirow{4}*{\rotatebox{90}{electricity}} & 96.0 & \uline{0.127$\pm$0.001} & 0.129 & 0.131 & 0.13 & \uline{0.127} & 0.128 & 0.129 & \textbf{0.126} & 0.129$\pm$0 \\ 
%         \multicolumn{1}{c|}{} & 192.0 & \textbf{0.145$\pm$0} & 0.149 & 0.149 & 0.148 & \textbf{0.145} & \uline{0.146} & 0.147 & \textbf{0.145} & \uline{0.146$\pm$0.001} \\ 
%         \multicolumn{1}{c|}{} & 336.0 & \textbf{0.156$\pm$0.001} & 0.16 & 0.161 & 0.161 & \textbf{0.156} & \textbf{0.156} & 0.159 & 0.164 & \uline{0.158$\pm$0.001} \\ 
%         \multicolumn{1}{c|}{} & 720.0 & \textbf{0.185$\pm$0.002} & 0.187 & 0.189 & \uline{0.186} & 0.187 & \textbf{0.185} & 0.189 & 0.193 & \uline{0.186$\pm$0.001} \\ 
%         \hline 
%         \multirow{4}*{\rotatebox{90}{traffic}} & 96.0 & \textbf{0.348$\pm$0.001} & 0.359 & 0.368 & 0.367 & \uline{0.35} & \textbf{0.348} & \uline{0.35} & 0.352 & 0.356$\pm$0.002 \\ 
%         \multicolumn{1}{c|}{} & 192.0 & \textbf{0.37$\pm$0.001} & 0.38 & 0.387 & 0.384 & 0.372 & \textbf{0.37} & 0.372 & \uline{0.371} & 0.377$\pm$0.003 \\ 
%         \multicolumn{1}{c|}{} & 336.0 & \textbf{0.379$\pm$0.003} & 0.392 & 0.395 & 0.394 & \textbf{0.379} & \uline{0.38} & \textbf{0.379} & 0.381 & 0.385$\pm$0.002 \\ 
%         \multicolumn{1}{c|}{} & 720.0 & \textbf{0.42$\pm$0.001} & 0.428 & 0.43 & 0.431 & \textbf{0.42} & \uline{0.421} & 0.422 & 0.425 & 0.424$\pm$0.001 \\ 
%         \hline 
%         \multirow{4}*{\rotatebox{90}{weather}} & 96.0 & \textbf{0.143$\pm$0} & \uline{0.144} & 0.145 & 0.147 & \uline{0.144} & \textbf{0.143} & \uline{0.144} & \uline{0.144} & 0.146$\pm$0.001 \\ 
%         \multicolumn{1}{c|}{} & 192.0 & \textbf{0.189$\pm$0} & \uline{0.19} & 0.191 & 0.194 & \textbf{0.189} & \textbf{0.189} & \uline{0.19} & \uline{0.19} & 0.191$\pm$0.001 \\ 
%         \multicolumn{1}{c|}{} & 336.0 & \textbf{0.239$\pm$0.001} & 0.241 & 0.242 & 0.266 & \uline{0.24} & \textbf{0.239} & 0.241 & 0.244 & 0.243$\pm$0.001 \\ 
%         \multicolumn{1}{c|}{} & 720.0 & \textbf{0.311$\pm$0.001} & 0.319 & 0.328 & 0.321 & \textbf{0.311} & \uline{0.316} & 0.319 & 0.32 & \uline{0.316$\pm$0.001} \\ 
%         \hline 
%         \multicolumn{9}{c|}{\textbf{\citsm-Overall-Best (SS) \% Improvement}} & \textbf{1.45\%}  & \textbf{1.41\%}  \\
%         \hline 
%     \end{tabular}
%     }
%     \caption{Self-Supervised(SS) MSE benchmarking}
%     \label{tab:fm-2-all}
% \end{table*}


\begin{table*}[t]
    % \setlength{\tabcolsep}{5pt}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        
        & FL  &  \multicolumn{3}{c|}{\makecell{\citsm-Best (SS) \\ Model Size: Default}}& \multicolumn{3}{c|}{\makecell{\citsm-Best (SS) \\ Model Size: Big}}& \makecell{\textbf{\citsm-}\\\textbf{Overall-Best (SS)}} & \makecell{PatchTST \\ (SS)}& \makecell{\citsm-\\Best} \\ \hline

        & & SAME & ALL & TL & SAME & ALL & TL & & & Supervised\\ \hline
        \multirow{4}*{\rotatebox{90}{Electricity}} & 96.0 & 0.129 & 0.131 & 0.13 & \uline{0.127} & 0.128 & 0.129 & \uline{0.127$\pm$0.001} & \textbf{0.126} & 0.129$\pm$0 \\ 
        \multicolumn{1}{c|}{} & 192.0 & 0.149 & 0.149 & 0.148 & \textbf{0.145} & \uline{0.146} & 0.147 & \textbf{0.145$\pm$0} & \textbf{0.145} & \uline{0.146$\pm$0.001} \\ 
        \multicolumn{1}{c|}{} & 336.0 & 0.16 & 0.161 & 0.161 & \textbf{0.156} & \textbf{0.156} & 0.159 & \textbf{0.156$\pm$0.001} & 0.164 & \uline{0.158$\pm$0.001} \\ 
        \multicolumn{1}{c|}{} & 720.0 & 0.187 & 0.189 & \uline{0.186} & 0.187 & \textbf{0.185} & 0.189 & \textbf{0.185$\pm$0.002} & 0.193 & \uline{0.186$\pm$0.001} \\ 
        \hline 
        \multirow{4}*{\rotatebox{90}{Traffic}} & 96.0 & 0.359 & 0.368 & 0.367 & \uline{0.35} & \textbf{0.348} & \uline{0.35} & \textbf{0.348$\pm$0.001} & 0.352 & 0.356$\pm$0.002 \\ 
        \multicolumn{1}{c|}{} & 192.0 & 0.38 & 0.387 & 0.384 & 0.372 & \textbf{0.37} & 0.372 & \textbf{0.37$\pm$0.001} & \uline{0.371} & 0.377$\pm$0.003 \\ 
        \multicolumn{1}{c|}{} & 336.0 & 0.392 & 0.395 & 0.394 & \textbf{0.379} & \uline{0.38} & \textbf{0.379} & \textbf{0.379$\pm$0.003} & 0.381 & 0.385$\pm$0.002 \\ 
        \multicolumn{1}{c|}{} & 720.0 & 0.428 & 0.43 & 0.431 & \textbf{0.42} & \uline{0.421} & 0.422 & \textbf{0.42$\pm$0.001} & 0.425 & 0.424$\pm$0.001 \\ 
        \hline 
        \multirow{4}*{\rotatebox{90}{Weather}} & 96.0 & \uline{0.144} & 0.145 & 0.147 & \uline{0.144} & \textbf{0.143} & \uline{0.144} & \textbf{0.143$\pm$0} & \uline{0.144} & 0.146$\pm$0.001 \\ 
        \multicolumn{1}{c|}{} & 192.0 & \uline{0.19} & 0.191 & 0.194 & \textbf{0.189} & \textbf{0.189} & \uline{0.19} & \textbf{0.189$\pm$0} & \uline{0.19} & 0.191$\pm$0.001 \\ 
        \multicolumn{1}{c|}{} & 336.0 & 0.241 & 0.242 & 0.266 & \uline{0.24} & \textbf{0.239} & 0.241 & \textbf{0.239$\pm$0.001} & 0.244 & 0.243$\pm$0.001 \\ 
        \multicolumn{1}{c|}{} & 720.0 & 0.319 & 0.328 & 0.321 & \textbf{0.311} & \uline{0.316} & 0.319 & \textbf{0.311$\pm$0.001} & 0.32 & \uline{0.316$\pm$0.001} \\ 
        \hline 
        \multicolumn{9}{c|}{\textbf{\citsm-Overall-Best (SS) \% Improvement}} & \textbf{1.45\%}  & \textbf{1.41\%}  \\
        \hline 
    \end{tabular}
    }
    \caption{Self-Supervised(SS) MSE benchmarking with varying data and model sizes}
    \label{tab:fm-2-all}
\end{table*}


% \begin{table}[htbp]
% \centering
% \setlength{\tabcolsep}{2pt}
% \scalebox{0.9}{
% \begin{tabular}{c|c|c|c|c|}
% \hline  
% Data & Forecast Length & LightTS & S4 & \textbf{\citsm-Best}  \\
% \hline
% ETTH1 & 336 & 0.466 & 1.407 & \textbf{0.421} \\ \hline
% ETTH1 & 720 & 0.542 & 1.162 & \textbf{0.444} \\ \hline
% ETTH2 & 336 & 0.497 & 1.98 & \textbf{0.357} \\ \hline
% ETTH2 & 720 & 0.739 & 2.65 & \textbf{0.395} \\ \hline
% Weather & 336 & 0.527 & 0.531 & \textbf{0.243} \\ \hline
% Weather & 720 & 0.554 & 0.578 & \textbf{0.316} \\ \hline
% \multicolumn{2}{c|}{\textbf{Relative \% improvement}}& \textbf{33.2} & \textbf{66.4} & \\ \hline
% \end{tabular}}
% \caption{LightTS and S4 MSE Benchmarking}
% \label{tab:lightts2}
% \end{table}




% % \linespread{1.2}
% \begin{table*}[t]
%         % \small
% 	\centering
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{cc|c|cc|cc|cc|cc|cc|ccc}
% 			\cline{2-15}
% 			&\multicolumn{2}{c|}{Models}& \multicolumn{2}{c|}{PatchTST}& \multicolumn{2}{c|}{FEDformer}& \multicolumn{2}{c|}{Autoformer}& \multicolumn{2}{c|}{Informer}& \multicolumn{2}{c|}{DLinear}& \multicolumn{2}{c}{\citsm-Best} \\
% 			\cline{2-15}
% 			&\multicolumn{2}{c|}{Metric}&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE\\
% 			\cline{2-15}
% 			&\multirow{4}*{\rotatebox{90}{Weather}}& 96    & \textbf{0.149} & \textbf{0.198} & \uline{0.152} & \uline{0.199} & 0.176 & 0.237 & 0.238 & 0.314 & 0.249 & 0.329 & 0.354$\pm$0.001 & 0.405$\pm$0.001 \\
%             &\multicolumn{1}{c|}{}& 192   & \textbf{0.194} & \textbf{0.241} & \uline{0.197} & \uline{0.243} & 0.220 & 0.282 & 0.275 & 0.329 & 0.325 & 0.370 & 0.419$\pm$0.001 & 0.434$\pm$0.001  \\
% 			\cline{2-15}
                
% 		\end{tabular}
% 	}
% 	\caption{result}
% 	\label{tab:supervised}
% \end{table*}
% % \linespread{1}




